Islands in the Gap: Intertwined Transport and Localization in Structurally Complex Materials

Localized waves in disordered one-dimensional materials have been studied for decades, including white-noise and correlated disorder, as well as quasi-periodic disorder. How these wave phenomena relate to those in crystalline (periodic ordered) materials---arguably the better understood setting---has been a mystery ever since Anderson discovered disorder-induced localization. Nonetheless, together these revolutionized materials science and technology and led to new physics far beyond the solid state. We introduce a broad family of structurally complex materials---chaotic crystals---that interpolate between these organizational extremes---systematically spanning periodic structures and random disorder. Within the family one can tune the degree of disorder to sweep through an intermediate structurally disordered region between two periodic lattices. This reveals new transport and localization phenomena reflected in a rich array of energy-dependent localization degree and density of states. In particular, strong localization is observed even with a very low degree of disorder. Moreover, markedly enhanced localization and delocalization coexist in a very narrow range of energies. Most notably, beyond the simply smoothed bands found in previous disorder studies, islands of transport emerge in band gaps and sharp band boundaries persist in the presence of substantial disorder. Finally, the family of materials comes with rather direct specifications of how to assemble the requisite material organizations.

==> cmechabbrev.tex <==
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator*{\argmax}{argmax}

% Abbreviations from CMPPSS:

\newcommand{\eM}     {\mbox{$\epsilon$-machine}\xspace}
\newcommand{\eMs}    {\mbox{$\epsilon$-machines}\xspace}
\newcommand{\EM}     {\mbox{$\epsilon$-Machine}\xspace}
\newcommand{\EMs}    {\mbox{$\epsilon$-Machines}\xspace}
\newcommand{\eT}     {\mbox{$\epsilon$-transducer}\xspace}
\newcommand{\eTs}    {\mbox{$\epsilon$-transducers}\xspace}
\newcommand{\ET}     {\mbox{$\epsilon$-Transducer}\xspace}
\newcommand{\ETs}    {\mbox{$\epsilon$-Transducers}\xspace}

% cryptic
\newcommand{\order}[1]{order\protect\nobreakdash-$#1$}
\newcommand{\Order}[1]{Order\protect\nobreakdash-$#1$}
\newcommand{\cryptic}[1]{$#1$\protect\nobreakdash-cryptic}
\newcommand{\Cryptic}[1]{$#1$\protect\nobreakdash-Cryptic}
\newcommand{\crypticity}[1]{$#1$\protect\nobreakdash-crypticity}
\newcommand{\Crypticity}[1]{$#1$\protect\nobreakdash-Crypticity}

% Processes and sequences

\newcommand{\Process}{\mathcal{P}}

\newcommand{\ProbMach}{\Prob_{\mathrm{M}}}
\newcommand{\Lmax}   { {L_{\mathrm{max}}}}
\newcommand{\MeasAlphabet}      {\mathcal{A}}
% Original symbol
%\newcommand{\MeasSymbol}   { {S} }
%\newcommand{\meassymbol}   { {s} }
% New symbol
\newcommand{\MeasSymbol}   { {X} }
\newcommand{\meassymbol}   { {x} }
\newcommand{\BiInfinity}        { \smash{\overleftrightarrow {\MeasSymbol}} }
\newcommand{\biinfinity}        { \smash{\overleftrightarrow {\meassymbol}} }
\newcommand{\Past}      { \smash{\overleftarrow {\MeasSymbol}} }
\newcommand{\past}      { \smash{\overleftarrow {\meassymbol}} }
\newcommand{\pastprime} { {\past}^{\prime}}
\newcommand{\Future}    { \smash{\overrightarrow{\MeasSymbol}} }
\newcommand{\future}    { \smash{\overrightarrow{\meassymbol}} }
\newcommand{\futureprime}       { \smash{\future^{\prime}} }
\newcommand{\PastPrime}     { \smash{\Past^{\prime}} }
\newcommand{\FuturePrime}       { \smash{\overrightarrow{\meassymbol}^\prime} }
\newcommand{\PastDblPrime}      { \smash{\overleftarrow{\meassymbol}^{\prime\prime}} }
\newcommand{\FutureDblPrime}{ \smash{\overrightarrow{\meassymbol}^{\prime\prime}} }
\newcommand{\pastL}     { \smash{\overleftarrow {\meassymbol}{}^L} }
\newcommand{\PastL}     { \smash{\overleftarrow {\MeasSymbol}{}^L} }
\newcommand{\PastLt}      { \smash{\overleftarrow {\MeasSymbol}_t^L} }
\newcommand{\PastLLessOne}{ \smash{\overleftarrow {\MeasSymbol}^{L-1}} }
\newcommand{\futureL}     { \smash{\overrightarrow{\meassymbol}{}^L} }
\newcommand{\FutureL}     { \smash{\overrightarrow{\MeasSymbol}{}^L} }
\newcommand{\FutureLt}    { \smash{\overrightarrow{\MeasSymbol}_t^L} }
\newcommand{\FutureLLessOne}{ \smash{\overrightarrow{\MeasSymbol}^{L-1}} }
\newcommand{\pastLprime}        { \smash{\overleftarrow {\meassymbol}^{L^\prime}} }
\newcommand{\futureLprime}      { \smash{\overrightarrow{\meassymbol}^{L^\prime}} }
\newcommand{\AllPasts}      { \smash{\overleftarrow{ {\rm {\bf \MeasSymbol}} } } }
\newcommand{\AllFutures}        { \smash{\overrightarrow{ {\rm {\bf \MeasSymbol}} } } }
\newcommand{\FutureSet} { \smash{\overrightarrow{\bf \MeasSymbol}} }

% Causal states and epsilon-machines
\newcommand{\CausalState}       { \mathcal{S} }
\newcommand{\CausalStatePrime}  { {\CausalState}^{\prime}}
\newcommand{\causalstate}       { \sigma }
\newcommand{\CausalStateSet}    { \boldsymbol{\CausalState} }
\newcommand{\AlternateState}    { \mathcal{R} }
\newcommand{\AlternateStatePrime}       { {\cal R}^{\prime} }
\newcommand{\alternatestate}    { \rho }
\newcommand{\alternatestateprime}       { {\rho^{\prime}} }
\newcommand{\AlternateStateSet} { \boldsymbol{\AlternateState} }
\newcommand{\PrescientState}    { \widehat{\AlternateState} }
\newcommand{\prescientstate}    { \widehat{\alternatestate} }
\newcommand{\PrescientStateSet} { \boldsymbol{\PrescientState}}
\newcommand{\CausalEquivalence} { {\sim}_{\epsilon} }
\newcommand{\CausalEquivalenceNot}      { {\not \sim}_{\epsilon}}

\newcommand{\NonCausalEquivalence}      { {\sim}_{\eta} }
\newcommand{\NextObservable}    { {\smash{\overrightarrow {\MeasSymbol}}^1} }
\newcommand{\LastObservable}    { {\smash{\overleftarrow {\MeasSymbol}}^1} }
%\newcommand{\Prob}             { {\rm P}}
\newcommand{\Prob}      {\Pr} % use standard command
\newcommand{\ProbAnd}   { {,\;} }
\newcommand{\LLimit}    { {L \rightarrow \infty}}
\newcommand{\Cmu}               {C_\mu}
\newcommand{\hmu}               {h_\mu}
\newcommand{\EE}                {{\bf E}}
\newcommand{\TI}                {{\bf T}}
\newcommand{\SyncI}        {{\bf S}}
\newcommand{\Measurable}{{\bf \mu}}

% Process Crypticity
\newcommand{\PC}                {\chi}

% Causal Irreversibility
\newcommand{\CI}                {\Xi}
\newcommand{\ReverseMap}        {r}
\newcommand{\ForwardMap}        {f}

% Abbreviations from IB:
% None that aren't already in CMPPSS

% Abbreviations from Extensive Estimation:
\newcommand{\EstCausalState}    {\widehat{\CausalState}}
\newcommand{\estcausalstate}    {\widehat{\causalstate}}
\newcommand{\EstCausalStateSet} {\boldsymbol{\EstCausalState}}
\newcommand{\EstCausalFunc}     {\widehat{\epsilon}}
\newcommand{\EstCmu}            {\widehat{\Cmu}}
\newcommand{\PastLOne}  {{\Past}^{L+1}}
\newcommand{\pastLOne}  {{\past}^{L+1}}

% Abbreviations from $\epsilon$-Transducers:
\newcommand{\InAlphabet}        { \mathcal{A}}
\newcommand{\insymbol}          { a}
\newcommand{\OutAlphabet}       { \mathcal{B}}
\newcommand{\outsymbol}         { b}
\newcommand{\InputSimple}       { X}
\newcommand{\inputsimple}       { x}
\newcommand{\BottleneckVar}     {\tilde{\InputSimple}}
\newcommand{\bottleneckvar}     {\tilde{\inputsimple}}
\newcommand{\InputSpace}        { \mathbf{\InputSimple}}
\newcommand{\InputBi}   { \overleftrightarrow {\InputSimple} }
\newcommand{\inputbi}   { \overleftrightarrow {\inputsimple} }
\newcommand{\InputPast} { \overleftarrow {\InputSimple} }
\newcommand{\inputpast} { \overleftarrow {\inputsimple} }
\newcommand{\InputFuture}       { \overrightarrow {\InputSimple} }
\newcommand{\inputfuture}       { \overrightarrow {\inputsimple} }
\newcommand{\NextInput} { {{\InputFuture}^{1}}}
\newcommand{\NextOutput}        { {\OutputFuture}^{1}}
\newcommand{\OutputSimple}      { Y}
\newcommand{\outputsimple}      { y}
\newcommand{\OutputSpace}       { \mathbf{\OutputSimple}}
\newcommand{\OutputBi}  { \overleftrightarrow{\OutputSimple} }
\newcommand{\outputbi}  { \overleftrightarrow{\outputsimple} }
\newcommand{\OutputPast}        { \overleftarrow{\OutputSimple} }
\newcommand{\outputpast}        { \overleftarrow{\outputsimple} }
\newcommand{\OutputFuture}      { \overrightarrow{\OutputSimple} }
\newcommand{\outputfuture}      { \overrightarrow{\outputsimple} }
\newcommand{\OutputL}   { {\OutputFuture}^L}
\newcommand{\outputL}   { {\outputfuture}^L}
\newcommand{\InputLLessOne}     { {\InputFuture}^{L-1}}
\newcommand{\inputLlessone}     { {\inputufutre}^{L-1}}
\newcommand{\OutputPastLLessOne}        {{\OutputPast}^{L-1}_{-1}}
\newcommand{\outputpastLlessone}        {{\outputpast}^{L-1}}
\newcommand{\OutputPastLessOne} {{\OutputPast}_{-1}}
\newcommand{\outputpastlessone} {{\outputpast}_{-1}}
\newcommand{\OutputPastL}       {{\OutputPast}^{L}}
\newcommand{\OutputLPlusOne}    { {\OutputFuture}^{L+1}}
\newcommand{\outputLplusone}    { {\outputfutre}^{L+1}}
\newcommand{\InputPastL}        {{\InputPast}^{L}}
\newcommand{\inputpastL}        {{\inputpast}^{L}}
\newcommand{\JointPast} {{(\InputPast,\OutputPast)}}
\newcommand{\jointpast} {{(\inputpast,\outputpast)}}
\newcommand{\jointpastone}      {{(\inputpast_1,\outputpast_1)}}
\newcommand{\jointpasttwo}      {{(\inputpast_2,\outputpast_2)}}
\newcommand{\jointpastprime} {{({\inputpast}^{\prime},{\outputpast}^{\prime})}}
\newcommand{\NextJoint} {{(\NextInput,\NextOutput)}}
\newcommand{\nextjoint} {{(\insymbol,\outsymbol)}}
\newcommand{\AllInputPasts}     { { \overleftarrow {\rm \InputSpace}}}
\newcommand{\AllOutputPasts}    { {\overleftarrow {\rm \OutputSpace}}}
\newcommand{\DetCausalState}    { {{\cal S}_D }}
\newcommand{\detcausalstate}    { {{\sigma}_D} }
\newcommand{\DetCausalStateSet} { \boldsymbol{{\CausalState}_D}}
\newcommand{\DetCausalEquivalence}      { {\sim}_{{\epsilon}_{D}}}
\newcommand{\PrescientEquivalence}      { {\sim}_{\widehat{\eta}}}
\newcommand{\FeedbackCausalState}       { \mathcal{F}}
\newcommand{\feedbackcausalstate}       { \phi}
\newcommand{\FeedbackCausalStateSet}    { \mathbf{\FeedbackCausalState}}
\newcommand{\JointCausalState}          { \mathcal{J}}
\newcommand{\JointCausalStateSet}       { \mathbf{\JointCausalState}}
\newcommand{\UtilityFunctional} { {\mathcal{L}}}
\newcommand{\NatureState}       { {\Omega}}
\newcommand{\naturestate}       { {\omega}}
\newcommand{\NatureStateSpace}  { {\mathbf{\NatureState}}}
\newcommand{\AnAction}  { {A}}
\newcommand{\anaction}  { {a}}
\newcommand{\ActionSpace}       { {\mathbf{\AnAction}}}

% Abbreviations from RURO:
\newcommand{\InfoGain}[2] { \mathcal{D} \left( {#1} || {#2} \right) }

% Abbreviations from Upper Bound:
\newcommand{\lcm}       {{\rm lcm}}
% Double-check that this isn't in the math set already!

% Abbreviations from Emergence in Space
\newcommand{\ProcessAlphabet}   {\MeasAlphabet}
\newcommand{\ProbEst}                   { {\widehat{\Prob}_N}}
\newcommand{\STRegion}                  { {\mathrm K}}
\newcommand{\STRegionVariable}          { K}
\newcommand{\stregionvariable}          { k}
\newcommand{\GlobalPast}                { \overleftarrow{G}}
\newcommand{\globalpast}                { \overleftarrow{g}}
\newcommand{\GlobalFuture}              { \overrightarrow{G}}
\newcommand{\globalfuture}              { \overrightarrow{g}}
\newcommand{\GlobalState}               { \mathcal{G}}
\newcommand{\globalstate}               { \gamma}
\newcommand{\GlobalStateSet}            { {\mathbf \GlobalState}}
\newcommand{\LocalPast}                 { \overleftarrow{L}}
\newcommand{\localpast}                 { \overleftarrow{l}}
\newcommand{\AllLocalPasts}             { \mathbf{\LocalPast}}
\newcommand{\LocalPastRegion}           { \overleftarrow{\mathrm L}}
\newcommand{\LocalFuture}               { \overrightarrow{L}}
\newcommand{\localfuture}               { \overrightarrow{l}}
\newcommand{\LocalFutureRegion}         { \overrightarrow{\mathrm L}}
\newcommand{\LocalState}                { \mathcal{L}}
\newcommand{\localstate}                { \lambda}
\newcommand{\LocalStateSet}             { {\mathbf \LocalState}}
\newcommand{\PatchPast}                 { \overleftarrow{P}}
\newcommand{\patchpast}                 { \overleftarrow{p}}
\newcommand{\PatchPastRegion}           { \overleftarrow{\mathrm P}}
\newcommand{\PatchFuture}               { \overrightarrow{P}}
\newcommand{\patchfuture}               { \overrightarrow{p}}
\newcommand{\PatchFutureRegion}         { \overrightarrow{\mathrm P}}
\newcommand{\PatchState}                { \mathcal{P}}
\newcommand{\patchstate}                { \pi}
\newcommand{\PatchStateSet}             { {\mathbf \PatchState}}
\newcommand{\LocalStatesInPatch}        {\vec{\LocalState}}
\newcommand{\localstatesinpatch}        {\vec{\localstate}}
\newcommand{\PointInstantX}             { {\mathbf x}}
% Galles's original LaTeX for the cond. indep. symbol follows:
\newcommand{\compos}{\mbox{$~\underline{~\parallel~}~$}}
\newcommand{\ncompos}{\not\hspace{-.15in}\compos}
\newcommand{\indep}                     { \rotatebox{90}{$\models$}}
\newcommand{\nindep}    {\not\hspace{-.05in}\indep}
\newcommand{\LocalEE}   {{\EE}^{loc}}
\newcommand{\EEDensity} {\overline{\LocalEE}}
\newcommand{\LocalCmu}  {{\Cmu}^{loc}}
\newcommand{\CmuDensity}        {\overline{\LocalCmu}}

%%%%%%%%%%% added by sasa
\newcommand{\FinPast}[1]        { \overleftarrow {\MeasSymbol} \stackrel{{#1}}{}}
\newcommand{\finpast}[1]        { \overleftarrow {\meassymbol}  \stackrel{{#1}}{}}
\newcommand{\FinFuture}[1]              { \overrightarrow{\MeasSymbol} \stackrel{{#1}}{}}
\newcommand{\finfuture}[1]              { \overrightarrow{\meassymbol} \stackrel{{#1}}{}}

\newcommand{\Partition} { \AlternateState }
\newcommand{\partitionstate}    { \alternatestate }
\newcommand{\PartitionSet}      { \AlternateStateSet }
\newcommand{\Fdet}   { F_{\rm det} }

\newcommand{\Dkl}[2] { D_{\rm KL} \left( {#1} || {#2} \right) }

\newcommand{\Period}    {p}

% To take into account time direction
\newcommand{\forward}{+}
\newcommand{\reverse}{-}
%\newcommand{\forwardreverse}{\:\!\diamond} % \pm
\newcommand{\forwardreverse}{\pm} % \pm
\newcommand{\FutureProcess}     { {\Process}^{\forward} }
\newcommand{\PastProcess}       { {\Process}^{\reverse} }
\newcommand{\FutureCausalState} { {\CausalState}^{\forward} }
\newcommand{\futurecausalstate} { \sigma^{\forward} }
\newcommand{\altfuturecausalstate}      { \sigma^{\forward\prime} }
\newcommand{\PastCausalState}   { {\CausalState}^{\reverse} }
\newcommand{\pastcausalstate}   { \sigma^{\reverse} }
\newcommand{\BiCausalState}             { {\CausalState}^{\forwardreverse} }
\newcommand{\bicausalstate}             { {\sigma}^{\forwardreverse} }
\newcommand{\FutureCausalStateSet}      { {\CausalStateSet}^{\forward} }
\newcommand{\PastCausalStateSet}        { {\CausalStateSet}^{\reverse} }
\newcommand{\BiCausalStateSet}  { {\CausalStateSet}^{\forwardreverse} }
\newcommand{\eMachine}  { M }
\newcommand{\FutureEM}  { {\eMachine}^{\forward} }
\newcommand{\PastEM}    { {\eMachine}^{\reverse} }
\newcommand{\BiEM}              { {\eMachine}^{\forwardreverse} }
\newcommand{\BiEquiv}   { {\sim}^{\forwardreverse} }
\newcommand{\Futurehmu} { h_\mu^{\forward} }
\newcommand{\Pasthmu}   { h_\mu^{\reverse} }
\newcommand{\FutureCmu} { C_\mu^{\forward} }
\newcommand{\PastCmu}   { C_\mu^{\reverse} }
\newcommand{\BiCmu}             { C_\mu^{\forwardreverse} }
\newcommand{\FutureEps} { \epsilon^{\forward} }
\newcommand{\PastEps}   { \epsilon^{\reverse} }
\newcommand{\BiEps}     { \epsilon^{\forwardreverse} }
\newcommand{\FutureSim} { \sim^{\forward} }
\newcommand{\PastSim}   { \sim^{\reverse} }
\newcommand{\FuturePC}  {\PC^{\forward}}
\newcommand{\PastPC}            {\PC^{\reverse}}
\newcommand{\BiPC}      {\PC^{\forwardreverse}}

% Used arrows for awhile, more or less confusing?
%\newcommand{\FutureCausalState}        { \overrightarrow{\CausalState} }
%\newcommand{\PastCausalState}  { \overleftarrow{\CausalState} }
%\newcommand{\eMachine} { M }
%\newcommand{\FutureEM} { \overrightarrow{\eMachine} }
%\newcommand{\PastEM}   { \overleftarrow{\eMachine} }
%\newcommand{\FutureCmu}        { \overrightarrow{\Cmu} }
%\newcommand{\PastCmu}  { \overleftarrow{\Cmu} }

%% time-reversing and mixed state presentation operators
\newcommand{\TR}{\mathcal{T}}
\newcommand{\MSP}{\mathcal{U}}
\newcommand{\one}{\mathbf{1}}

%% added for RURO2
%% Note that it will always be typesett in math mode.
%% Example usage:
%%    The 3-block entropy is \BE[t]{3}.
%%    The 3-block-state entropy from $t=0$ is $\BSE{3}$.
%%
%% The optional argument specifies the start time, defaulting to t=0.
%% The mandatory argument specifies the length of the block (not the stop time).
\newcommand{\lastindex}[2]{
  \edef\tempa{0}
  \edef\tempb{#2}
  \ifx\tempa\tempb
    % if the length is 0, then the final time equals the start time
    \edef\tempc{#1}
  \else
    % if the start time is different from zero, then we show the sum
    \edef\tempa{0}
    \edef\tempb{#1}
    \ifx\tempa\tempb
      \edef\tempc{#2}
    \else
      \edef\tempc{#1+#2}
    \fi
  \fi
  \tempc
}
\newcommand{\BE}[2][0]{
  \ensuremath{H[\MeasSymbol_{#1}^{#2}]}
}
\newcommand{\BSE}[2][0]{
  \ensuremath{H[\MeasSymbol_{#1}^{#2},\CausalState_{\lastindex{#1}{#2}}]}%
}
\newcommand{\SBE}[2][0]{
  \ensuremath{H[\CausalState_{#1},\MeasSymbol_{#1}^{#2}]}
}
\newcommand{\SBSE}[2][0]{
  \ensuremath{H[\CausalState_{#1},\MeasSymbol_{#1}^{#2},
                \CausalState_{\lastindex{#1}{#2}}]}
}
\newcommand{\AltSBE}[2][0]{
  \ensuremath{H[\AlternateState_{#1},\MeasSymbol_{#1}^{#2}]}
}
\newcommand{\AltBSE}[2][0]{
  \ensuremath{H[\MeasSymbol_{#1}^{#2},\AlternateState_{\lastindex{#1}{#2}}]}
}
\newcommand{\AltSBSE}[2][0]{
  \ensuremath{H[\AlternateState_{#1},\MeasSymbol_{#1}^{#2},
                \AlternateState_{\lastindex{#1}{#2}}]}
}

\newcommand{\GI}{\varphi}
\newcommand{\OI}{\zeta}
% cryptic, gauge, oracular, Markov, and synchronization
\newcommand{\COrder}{k_{\PC}}
\newcommand{\GOrder}{k_{\GI}}
\newcommand{\OOrder}{k_{\OI}}
\newcommand{\MOrder}{R}
\newcommand{\SOrder}{k_{\SI}}


%% Added to standardize the order of causal states
%% Example usage:
%%    $\BiCmu = H[\CSjoint] = H[\CSjoint[,]]$
%%    $\EE = I[\CSjoint[:]] = I[\CSjoint[;]]$
\newcommand{\CSjoint}[1][,]{
   \edef\tempa{:}
   \edef\tempb{#1}
   \ifx\tempa\tempb
      % arg1 was a colon, insert a small negative space
      \ensuremath{\FutureCausalState\!#1\PastCausalState}
   \else
      % arg1 was not a colon, usually a comma or semicolon
      \ensuremath{\FutureCausalState#1\PastCausalState}
   \fi
}
\newcommand{\CSjointKL}[3][,]{
   \edef\tempa{:}
   \edef\tempb{#1}
   \ifx\tempa\tempb
      % arg1 was a colon, insert a small negative space
      \ensuremath{\FutureCausalState_{#2}\!#1\PastCausalState_{#3}}
   \else
      % arg1 was not a colon, usually a comma or semicolon
      \ensuremath{\FutureCausalState_{#2}#1\PastCausalState_{#3}}
   \fi
}


%% (cje)
%% Provide a command \ifpm which is true when \pm
%% is meant to be understood as "+ or -", opposed
%% to "bidirectional". This differs from the usage
%% in TBA.  Essentially, if \forwardreverse is defined
%% as something different, perhaps a \diamond, then
%% we are free to interpret \pm as "+ or -".
\newif\ifpm
\edef\tempa{\forwardreverse}
\edef\tempb{\pm}
\ifx\tempa\tempb
   \pmfalse
\else
   \pmtrue
\fi


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Metric quantities of information generation, eg anatomy of a bit

\newcommand{\metric}[1] {\ensuremath{#1_\mu}\xspace}

\renewcommand{\hmu}{\metric{h}}
\newcommand{\rhomu}{\metric{\rho}}
\newcommand{\rmu}{\metric{r}}
\newcommand{\bmu}{\metric{b}}
\newcommand{\qmu}{\metric{q}}
\newcommand{\wmu}{\metric{w}}
\newcommand{\imu}{\metric{i}}
\newcommand{\sigmamu}{\metric{\sigma}}

\newcommand{\himc}{\ensuremath{h_{imc}}\xspace}
\newcommand{\pee}{\ensuremath{pee}\xspace} % parallel edge entropy

\newcommand{\ExE}[1] {\ensuremath{\EE_{#1}}\xspace}

\newcommand{\EER}{\ExE{R}}
\newcommand{\EEB}{\ExE{B}}
\newcommand{\EEQ}{\ExE{Q}}
\newcommand{\EEW}{\ExE{W}}
\newcommand{\EI}{\mathbf{I}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Time series, using the python-esque notation

\newcommand{\MS} [2] {\ensuremath{\MeasSymbol_{#1:#2}}\xspace}
\newcommand{\ms} [2] {\ensuremath{\meassymbol_{#1:#2}}\xspace}

\renewcommand{\Past}       {\MS{}{0}}
\newcommand{\Present}      {\ensuremath{\MeasSymbol_{0}}\xspace}
\renewcommand{\Future}     {\MS{0}{}}
\newcommand{\LPresent} [1] {\MS{0}{#1}}
\newcommand{\LFuture}  [1] {\MS{#1}{}}

\renewcommand{\past}       {\ms{}{0}}
\newcommand{\present}      {\ensuremath{\meassymbol_{0}}\xspace}
\renewcommand{\future}     {\ms{0}{}}
\newcommand{\lpresent} [1] {\ms{0}{#1}}
\newcommand{\lfuture}  [1] {\ms{#1}{}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Causal states

\newcommand{\FCS}{\CausalState^\forward\xspace}
\newcommand{\RCS}{\CausalState^\reverse\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Others

\newcommand{\half}{\ensuremath{\nicefrac{1}{2}}}

\newcommand{\Language} {\ensuremath{\mathcal{L}}\xspace}
\newcommand{\Lsync} {\Language_{\mathrm{sync}}\xspace}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% mathclap, in case someone doesn't have mathtools

% TUGboat, Volume 0 (2001), No. 0
% http://math.arizona.edu/~aprl/publications/mathclap/perlis_mathclap_24Jun2003.pdf
% For comparison, here are the existing overlap macros:
% \def\llap#1{\hbox to 0pt{\hss#1}}
% \def\rlap#1{\hbox to 0pt{#1\hss}}
%
% These are provided by mathtools
%
\ifcsname mathclap\endcsname
  \relax
\else
  \def\clap#1{\hbox to 0pt{\hss#1\hss}}
  \def\mathllap{\mathpalette\mathllapinternal}
  \def\mathrlap{\mathpalette\mathrlapinternal}
  \def\mathclap{\mathpalette\mathclapinternal}
  \def\mathllapinternal#1#2{%
    \llap{$\mathsurround=0pt#1{#2}$}}
  \def\mathrlapinternal#1#2{%
    \rlap{$\mathsurround=0pt#1{#2}$}}
  \def\mathclapinternal#1#2{%
    \clap{$\mathsurround=0pt#1{#2}$}}
\fi


==> infotheory.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Information theory macros

% functions
\newcommand{\op}  [2]   {\ensuremath{\operatorname{#1}\left[#2\right]}\xspace}

\renewcommand{\H} [1]   {\op{H}{#1}}
\newcommand{\I}   [1]   {\op{I}{#1}}
\newcommand{\T}   [1]   {\op{T}{#1}}
\newcommand{\R}   [1]   {\op{R}{#1}}
\newcommand{\B}   [1]   {\op{B}{#1}}
\newcommand{\K}   [1]   {\op{K}{#1}}

% operators on random variables
\newcommand{\meet}      {\curlywedge}
\newcommand{\join}      {\curlyvee}
\newcommand{\iless}     {\preceq}
\newcommand{\imore}     {\succeq}
\newcommand{\ieq}       {\cong}
\newcommand{\mss}       {\downrightarrow}

